Search for top-squark pair production in final states with one lepton, jets, and missing transverse momentum using 36 fb$^{-1}$ of $\sqrt{s}=13$ TeV $pp$ collision data with the ATLAS detector

The results of a search for the direct pair production of top squarks, the supersymmetric partner of the top quark, in final states with one isolated electron or muon, several energetic jets, and missing transverse momentum are reported. The analysis also targets spin-0 mediator models, where the mediator decays into a pair of dark-matter particles and is produced in association with a pair of top quarks. The search uses data from proton-proton collisions delivered by the Large Hadron Collider in 2015 and 2016 at a centre-of-mass energy of $\sqrt{s}=13$ TeV and recorded by the ATLAS detector, corresponding to an integrated luminosity of 36 fb$^{-1}$. A wide range of signal scenarios with different mass-splittings between the top squark, the lightest neutralino and possible intermediate supersymmetric particles are considered, including cases where the W bosons or the top quarks produced in the decay chain are off-shell. No significant excess over the Standard Model prediction is observed. The null results are used to set exclusion limits at 95% confidence level in several supersymmetry benchmark models. For pair-produced top-squarks decaying into top quarks, top-squark masses up to 940 GeV are excluded. Stringent exclusion limits are also derived for all other considered top-squark decay scenarios. For the spin-0 mediator models, upper limits are set on the visible cross-section.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new".
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to rmeove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_latexmk instead of run_pdflatex to use latexmk to compile.

# If you have to run latex rather than pdflatex adjust the dependencies of %.dvi target
#   and use the command "make run_latex" to compile.
# Specify dvipdf or dvips as the run_latex dependency,
#   depending on which you want to use.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2016
LATEX    = latex
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
DVIPS    = dvips
DVIPDF   = dvipdf

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = paper
#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figures
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex
# Use latexmk instead to compile
# default: run_latexmk

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover auxmat
.PHONY: clean cleanpdf help

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.tex bibtex/bib/*.bib
%.pdf:	%.tex *.tex texfiles/*.tex *.bib
	$(PDFLATEX) $<
	rm -rf `biber --cache`
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex \
	  >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

auxmat:
	sed s/atlas-document/$(BASENAME)/ template/atlas-auxmat.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-auxmat.tex

newdocument:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newdocumenttexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' | \
	  sed 's/\\newcommand\*{\\ATLASLATEXPATH}{latex\/}/% \\newcommand\*{\\ATLASLATEXPATH}{latex\/}/' | \
	  sed 's/% \\newcommand\*{\\ATLASLATEXPATH}{}/\\newcommand\*{\\ATLASLATEXPATH}{}/' \
	  >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex; \
	fi

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	# touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

run_latex: dvipdf

# Targets if you run latex instead of pdflatex
dvipdf:	$(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress $<
	@echo "Made $(basename $<).pdf"

dvips:	$(BASENAME).dvi
	$(DVIPS) $<
	@echo "Made $(basename $<).ps"

# Specify dependencies for running latex
#%.dvi:	%.tex tex/*.tex bibtex/bib/*.bib
%.dvi:	%.tex *.tex texfiles/*.tex *.bib
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $<
	$(BIBTEX) $<

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for auxiliary material give the commands:"
	@echo "make auxmat [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-auxmat"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanps  to clean output PS files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx \
		*.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-auxmat.pdf

cleanps:
	-rm $(BASENAME).ps 
	-rm $(BASENAME)-draft-cover.ps $(BASENAME)-preprint-cover.ps
	-rm $(BASENAME)-auxmat.ps

cleanall: clean cleanpdf cleanps cleanepstopdf

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^


==> acknowledgements/Makefile <==
# Makefile for creating ATLAS Acknowledegments

TEXLIVE  = 2016
PDFLATEX = pdflatex
BIBTEX   = biber

BASENAME = Acknowledgements-main

.PHONY: clean cleanpdf

run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Change TeX Live version
texlive: $(BASENAME).tex
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  echo "Changing texlive value in $<"; \
	  sed -i'.bak' 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' $<; \
	else echo "Invalid value for TEXLIVE: $(TEXLIVE)"; fi; \

# Change biblatex backend
bibtex: $(BASENAME).tex
	if [ $(BIBTEX) = 'biber' -o $(BIBTEX) = 'bibtex' ]; then \
	  echo "Changing biblatex backend in $<"; \
	  sed -i'.bak' -e 's/backend=biber/backend=$(BIBTEX)/' -e 's/backend=bibtex/backend=$(BIBTEX)/' $<; \
	else echo "Invalid value for BIBTEX: $(BIBTEX)"; fi; \

# Standard LaTeX targets
$(BASENAME).pdf: $(BASENAME).tex
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<

%.bbl: %.tex *.bib
	$(PDFLATEX) $*
	$(BIBTEX) $*

clean:
	-rm *.dvi *.toc *.aux *.log *.out *.blg *.bbl *.bcf *-blx.bib \
	 *.run.xml *.synctex.gz *~ *.fls *.fdb_latexmk .*.lb spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf

cleanall: clean cleanpdf


==> texfiles/bkg_bC2x_CR.tex <==
\begin{table}[htbp]
  \centering
  \caption{
  Overview of the selections for the $\bCdiag$ and $\bCmed$ signal regions as well as the associated control and validation regions. The control regions include the semi-leptonic \ttbar\ control region (T1LCR), the dileptonic \ttbar\ control region (T2LCR), the $W$+jets control region (WCR), and the single-top $Wt$ control region (STCR).  The validation regions include the semi-leptonic \ttbar\ validation region (T1LVR), the dileptonic \ttbar\ validation region (T2LVR), and the $W$+jets validation region (WVR). List values are provided in between parentheses and square brackets denote intervals. 
  The veto on the reclustered hadronic $W$ boson candidate is satisfied for events where no reclustered jet candidate is found, or where the mass of the hadronic top-quark (\mTopRecluster) is below the specified tag threshold. For the WCR, $\DeltaR$($b_1$,$b_2$) $<1.2$ is not required when the event has only one $b$-tagged jet.
  The selection of the $\ttbar+Z$ control region (TZCR) is detailed in Section~\ref{subsec:ttZ}.
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | ccccc |}
    \hline
                                                &    \bCdiag       &        T1LCR/VR      &     T2LCR/VR     &         WCR/VR       &         STCR      \\ \hline
                Preselection                                & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)         & ($\ge4$,~$\ge2$) & ($\ge4$,~$\ge2$)     & ($\ge4$,~$\ge2$) & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge2$)  \\
    Jet $\pt $ \,[\GeV]           & \multicolumn{5}{ c |}{ $>(75~75~75~30)$ } \\
    $b$-tagged jet $\pt $ \,[\GeV]         & $>(30~30)$       & $>(30~30)$         & $>(30~30)$       & $>(30~-)$           & $>(30~30)$       \\
    \hline
    \met \,[\GeV]                         & \multicolumn{5}{ c |}{ $>230$} \\
    \HTmissSig                     & $>13$             & $>13$            & $>10$       & $>13$              & $>10$          \\ 
    \mt \,[\GeV]                 & $>180$          & $[30,90]$ / $[90,120]$ & $>120$        & $[30,90]$ / $[90,120]$ & $[30,120]$       \\
    \amtTwo  \,[\GeV]            & $>175$          & $<200$         & $<200$ / $<130$    & $>200$           & $>200$       \\
    $\minDeltaPhi(i=1,2)$                  & \multicolumn{5}{ c |}{ $>0.7$ } \\ 
    \mWRecluster \,[\GeV]          & $>50$           & $>50$            & $W$ veto / $>50$   & $W$ veto            & $W$ veto              \\
    $\DeltaR(b_1,b_2)$           & --               & --                   & --               & $<1.2$               & $>1.2$            \\
    Lepton charge                               & --               & --                   & --               & $=+1$                & --            \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$              & \multicolumn{5}{ c |}{$>0.4$}    \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]       & \multicolumn{5}{ c |}{$>80$}     \\ 
    \hline \hline
                                                &    \bCmed        &        T1LCR/VR      &     T2LCR/VR     &         WCR/VR       &         STCR      \\ \hline
                Preselection                                & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)         & ($\ge4$,~$\ge2$) & ($\ge4$,~$\ge2$)     & ($\ge4$,~$\ge1$) & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge2$)  \\
    Jet $\pt >$ \,[\GeV]           & \multicolumn{5}{ c |}{ $>(200~140~25~25)$  } \\ 
    $b$-tagged jet $\pt >$ \,[\GeV]       & $>(140~140)$     & $>(140~140)$        & $>(140~-)$    & $>(140~-)$          & $>(140~140)$      \\
    \hline
    \met \,[\GeV]                         & \multicolumn{5}{ c |}{ $>230$} \\
    \HTmissSig               & {$>10$}           & $>10$            & $>10$          & $>10$              & $>6$          \\
    \mt \,[\GeV]                 & $>120$           & $[30,90]$ / $[90,120]$ & $>120$       & $[30,90]$ / $[90,120]$  & $[30,120]$       \\
    \amtTwo  \,[\GeV]            & {$>300$}          & $<200$         & $<200$ / $<130$   & $>200$           & $>200$       \\
    $\minDeltaPhi(i=1,2)$                  & \multicolumn{5}{ c |}{ $>0.9$ } \\
    \mWRecluster \,[\GeV]          & $>50$         & $>50$            & $W$ veto / $>50$  & $W$ veto            & $W$ veto              \\
    $\DeltaR(b_1,b_2)$           & --               & --                   & --              & $<1.2$             & $>1.2$            \\
    Lepton charge                               & --               & --                   & --              & $=+1$                 & --                \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$              & \multicolumn{5}{ c |}{$>0.4$}    \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]       & \multicolumn{5}{ c |}{$>80$}     \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_bC2x}
\end{table}

\begin{table}[htbp]
  \centering
  \caption{
  Overview of the selections for the $\bCbv$ signal region, as well as the associated control regions for \ttbar\ (TCR) and $W$+jets (WCR), and the validation regions targeting \ttbar\ (TVR) and $W$+jets (WVR) backgrounds. List values are provided in between parentheses and square brackets denote intervals. 
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | ccc |}
    \hline
    \hline
                                              &  \bCbv       &        TCR/VR        &      WCR/VR           \\ \hline
                Preselection                              &  \multicolumn{3}{ c |}{high-\met\ preselection} \\ \hline
      Lepton \pt \, [\GeV]                      &  \multicolumn{3}{ c |}{ $>60$ }                                  \\ 
      Number of (jets,~$b$-tags)             &  ($\ge2$,~$=0$)    & ($\ge2$,~$\ge1$)     & ($\ge2$,~$=0$)      \\
      Jet $\pt$ \,[\GeV]                        &  \multicolumn{3}{ c |}{ $>(120~80)$}                              \\
    \hline
      \met \,[\GeV]                             &  \multicolumn{3}{ c |}{ $>360$ }                                   \\ 
      \HTmissSig                                &  \multicolumn{3}{ c |}{ $>16$ }                                    \\
      \mt \,[\GeV]                               &  $>200$             & $[30,90$] / $[90,120]$ & $[30,90]$ / $[90,120]$  \\
      $\minDeltaPhi(i=1)$                       &  \multicolumn{3}{ c |}{ $>2.0$ }                                   \\ 
      $\minDeltaPhi(i=2)$                       &  \multicolumn{3}{ c |}{ $>0.8$ }                                   \\ 
      $\dPMETlep$                          &  $>1.2$             & $-$                  & $-$                   \\
      $\mWRecluster$ \,[\GeV]                   &  \multicolumn{3}{ c |}{ $[70,100]$ }                               \\ 
        $|\Delta\phi(j_{1,2},\Ptmiss)|$            &  \multicolumn{3}{ c |}{$>0.4$}    \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_bCbv}
\end{table}


==> texfiles/bkg_bCsoft_CR.tex <==
\begin{table}[t!]
  \centering
  \caption{Overview of the selections for the $\bCsoftdiag$ and $\bffN$ signal regions, as well as the associated control regions for \ttbar\ (TCR) and $W$+jets (WCR), and the validation regions targeting \ttbar\ (TVR) and $W$+jets (WVR) backgrounds. List values are provided in between parentheses and square brackets denote intervals. 
  The veto on the reclustered hadronic top-quark candidate is satisfied for events where no reclustered jet candidate is found, or where the mass of the hadronic top-quark (\mTopRecluster) is below a certain threshold. The leading jet is required not to be $b$-tagged in all regions.
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | ccc |}
                \hline
    \hline
                                      & $\bCsoftdiag$/$\bffN$ & TCR/VR                & WCR/VR               \\ \hline
                Preselection                            & \multicolumn{3}{ c |}{soft-lepton preselection}                   \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge2$,~$\ge1$)  & ($\ge2$,~$\ge1$)      & ($\ge2$,~$=1$)        \\
    Jet $\pt$ \,[\GeV]       & \multicolumn{3}{ c| }{$(120~25)$}                                  \\
    \hline
    \met \,[\GeV]                     & \multicolumn{3}{ c| }{$>300$}                                      \\
    \mt \,[\GeV]                       & $<50$ / $<160$       & $<160$                & $<160$                \\
    $\pt^{\ell}$/$\met$              & $<0.02$       & $[0.03,0.10]$ / $<0.03$ & $[0.03,0.10]$ / $<0.03$ \\
    \mTopRecluster \,[\GeV]                 & top veto       & $>150$                & top veto              \\
    \dphiBPtmissMin                & $<1.5$        & $<1.5$               & $>1.5$                \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{3}{ c |}{$>0.4$}    \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_bCsoft_diag}
\end{table}

\begin{table}[htbp]
  \centering
  \caption{
  Overview of the selections for the $\bCsoftmed$ and $\bCsofthigh$ signal regions, as well as the associated control regions for \ttbar\ (TCR) and $W$+jets (WCR), and the validation regions targeting \ttbar\ (TVR) and $W$+jets (WVR) backgrounds. 
  List values are provided in between parentheses and square brackets denote intervals. The soft-lepton preselection as described in Table~\ref{tab:preselection} is applied to the signal regions. 
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | cccc |}
                \hline
    \hline
                                      & \bCsoftmed        & TCR/VR           & WCR/VR        & STCR/VR             \\ \hline
                Preselection                            & \multicolumn{4}{ c |}{soft-lepton preselection}                                  \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge3$,~$\ge2$)  & ($\ge3$,~$\ge2$) & ($\ge3$,~$=1$)      & ($\ge3$,~$\ge2$)    \\
    Jet $\pt $ \,[\GeV]       & \multicolumn{4}{ c |}{$>(120~60~40~25)$}                                          \\
    $b$-tagged jet $\pt$ \,[\GeV]           & $>(120~60)$       & $>(120~60)$      & $>120$              & $>(120~60)$          \\
    \hline
    \met \,[\GeV]                     & \multicolumn{4}{ c |}{$>230$}                                                    \\
    \mt \,[\GeV]                      & \multicolumn{4}{ c |}{$>160$}                                                    \\
    $\pt^W$ \,[\GeV]                      & \multicolumn{4}{ c |}{$>400$}                                                    \\
    $\pt^{\ell}$/$\met$              & $<0.03$       & $>0.03$ / $<0.03$  & $>0.20$ / $[0.1,0.2]$ & $>0.20$ / $[0.1,0.2]$ \\
                \amtTwo  \,[\GeV]                       & $>200$            & $<200$           & $>200$              & $>200$              \\
    \dphiBPtmissMin                & $>0.8$        & --          & $[0.8,2.5]$         & $>0.8$              \\
                $\Delta R(b_1,b_2)$                     & --                & --               & --                  & $>1.2$              \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{4}{ c |}{$>0.4$}    \\ 
    \hline \hline
                                      & \bCsofthigh       & TCR/VR           & WCR/VR        & STCR/VR             \\ \hline
                Preselection                            & \multicolumn{4}{ c |}{soft-lepton preselection}                                  \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge2$,~$\ge2$)  & ($\ge2$,~$\ge2$) & ($\ge2$,~$=1$)      & ($\ge2$,~$\ge2$)    \\
    Jet $\pt$ \,[\GeV]       & \multicolumn{4}{ c |}{$>(100~100)$}                                               \\
    $b$-tagged jet $\pt$ \,[\GeV]     & \multicolumn{4}{ c |}{$>(100~100)$}                                               \\
    \hline
    \met \,[\GeV]                     & \multicolumn{4}{ c |}{$>230$}                                                    \\
    \mt \,[\GeV]                      & \multicolumn{4}{ c |}{$>160$}                                                    \\
    $\pt^W$ \,[\GeV]                      & \multicolumn{4}{ c |}{$>500$}                                                    \\
    $\pt^{\ell}$/$\met$              & $<0.03$       & $>0.10$ / $<0.10$  & $[0.1,0.4]$ / $<0.10$ & $>0.30$ / $[0.1,0.3]$ \\
                \amtTwo  \,[\GeV]                       & $>300$            & $<300$           & $>300$              & $>300$              \\
    \dphiBPtmissMin                     & \multicolumn{4}{ c |}{$>0.4$}                                                    \\
                $\Delta R(b_1,b_2)$                     & $>0.8$            & $>0.8$           & --                  & $>0.8$              \\
                $\DeltaR(b,\ell)$                       & --                & --               & $>0.8$              & -- \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{4}{ c |}{$>0.4$}    \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_bCsoft}
\end{table}



==> texfiles/bkg_bWN_CR.tex <==
\begin{table}[htbp]
  \centering
  \caption{Overview of the selections for the \bWN\ signal region and associated CR. List values are provided in between parentheses and square brackets denote intervals. 
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | cc |}
                \hline
    \hline
                                & \bWN           & TCR/VR \\ \hline
                Preselection                            & \multicolumn{2}{ c |}{high-\met\ preselection} \\ \hline
                Number of (jets,~$b$-tags)              & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge1$)        \\
    Jet $\pt$  \,[\GeV]       & \multicolumn{2}{ c |}{$>(50~25~25~25)$}        \\
                \hline
                \met \,[\GeV]                           & $>300$               & $>230$                  \\
                \mt \,[\GeV]                            & $>130$               & $>130$                  \\
                \amtTwo  \,[\GeV]                       & $<110$               & $[130,170]$ / $[110,130]$ \\
                \dPMETlep                               & $<2.5$               & $>2.5$                  \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{2}{ c |}{$>0.4$}    \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]   & \multicolumn{2}{ c |}{$>80$}     \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_bWN}
\end{table}



==> texfiles/bkg_tN_diag_CR.tex <==
\begin{table}[htbp]
        \centering
        \caption{Overview of signal region and control region (CR) definitions for the BDT analyses targeting the compressed bino LSP scenarios. The selections described in Table~\ref{tab:SRs_tN_diag_low_high} are applied, except for the BDT score. 
  Square brackets denote intervals.
  }
        \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | c | c c | c c c|}
                \hline
                \hline
                Signal Region & \tNdiaglow   & \multicolumn{2}{c|}{\tNdiagmed} & \multicolumn{3}{c|}{\tNdiaghigh} \\ 
                BDT score &  $\geq 0.55$ &  \multicolumn{2}{c|}{$\geq 0.4$}  &  \multicolumn{3}{c|}{$\geq 0.6$} \\
                \hline
                Associated CRs  &  TCR & TCR1 & TCR2  &  TCR1 & TCR2 & TCR3 \\
                BDT score &  $[-1,\ 0.1]$ & $[-1,\ -0.4]$ & $[-0.4,\ 0.4]$  &  $[-1,\ -0.5]$ & $[-0.5,\ 0]$ & $[0,\ 0.4]$ \\
                \hline \hline
        \end{tabular*}
}
}
        \label{tab:BDT_CR_definitions}
\end{table}


==> texfiles/bkg_toptag_CR.tex <==
\begin{table}[htbp]
  \centering
  \caption{
  Overview of the selections for the $\tNmed$ and $\tNhigh$ signal regions as well as the associated control and validation regions. The control regions include the semi-leptonic \ttbar\ control region (T1LCR), the dileptonic \ttbar\ control region (T2LCR), the $W$+jets control region (WCR), and the single-top $Wt$ control region (STCR).  The validation regions include the semi-leptonic \ttbar\ validation region (T1LVR), the dileptonic \ttbar\ validation region (T2LVR), and the $W$+jets validation region (WVR). List values are provided in between parentheses and square brackets denote intervals. 
  The veto on the reclustered hadronic top-quark candidate is satisfied for events where no reclustered jet candidate is found, or where the mass of the hadronic top-quark (\mTopRecluster) is below the specified tag threshold. For the WCR, $\DeltaR$($b_1$,$b_2$) $<1.2$ is not required when the event has only one $b$-tagged jet.
  The selection of the $\ttbar+Z$ control region (TZCR) is detailed in Section~\ref{subsec:ttZ}.
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | ccccc |}
                \hline
    \hline
                                      & \tNmed        & T1LCR/VR             & T2LCR/VR         & WCR/VR                 & STCR \\ \hline
                Preselection                            & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge4$,~$\ge1$)  & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge1$) & ($\ge4$,~$\ge1$)      & ($\ge4$,~$\ge2$) \\
    Jet $\pt$ \,[\GeV]       & \multicolumn{5}{ c |}{$>(60~50~40~40)$} \\
    \hline
    \met \,[\GeV]                     & \multicolumn{5}{ c |}{$>250$} \\
    \perpmet \,[\GeV]                     & \multicolumn{5}{ c |}{$>230$} \\
    \mt \,[\GeV]                       & $>160$       & $[30,90]$ / $[90,120]$ & $>120$           & $[30,90]$ / $[90,120]$  & $[30,120]$ \\
    \HTmissSig                        & $>14$       & $>10$              & $>10$            & $>10$                 & $>10$ \\
    \mTopRecluster \,[\GeV]                 & $>150$       & $>150$               & top veto / $>150$  & top veto              & top veto \\
    \amtTwo \,[\GeV]                        & $>175$       & $<200$               & $<200$ / $<130$    & $>200$                & $>200$ \\
    $\DeltaR(b,\ell)$              & $<2.0$       & --                   & --               & --                    & -- \\
    $\DeltaR$($b_1$,$b_2$)             & --               & --                   & --               & $<1.2$                & $>1.2$ \\
    Lepton charge                     & --             & --              & --               & $+1$                  & -- \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{5}{ c |}{$>0.4$}    \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]   & \multicolumn{5}{ c |}{$>80$}     \\ 
    \hline \hline
                                       & \tNhigh        & T1LCR/VR       & T2LCR/VR         & WCR/VR                 & STCR \\ \hline
                Preselection                            & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge4$,~$\ge1$)  & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge1$) & ($\ge4$,~$\ge1$)      & ($\ge4$,~$\ge2$) \\
    Jet $\pt$ \,[\GeV]       & \multicolumn{5}{ c |}{$>(100~80~50~30)$} \\
    \hline
    \met \,[\GeV]                     & $>550$       & $>350$              & $>350$           & $>350$                & $>350$ \\
    \mt \,[\GeV]                       & $>160$       & $[30,90]$ / $[90,120]$ & $>120$           & $[30,90]$ / $[90,120]$  & $[30,120]$ \\
    \HTmissSig                        & $>27$       & $>10$              & $>10$            & $>10$                 & $>10$ \\
    \mTopRecluster \,[\GeV]                 & $>130$       & $>130$               & top veto / $>130$  & top veto              & top veto \\
    \amtTwo \,[\GeV]                        & $>175$       & $<200$               & $<200$ / $<130$    & $>200$                & $>200$ \\
    $\DeltaR(b,\ell)$              & $<2.0$       & --                   & --               & --                    & -- \\
    $\DeltaR$($b_1$,$b_2$)             & --               & --                   & --               & $<1.2$                & $>1.2$ \\
    Lepton charge                     & --             & --              & --               & $+1$                  & -- \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{5}{ c |}{$>0.4$}    \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]   & \multicolumn{5}{ c |}{$>80$}     \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_tN}
\end{table}

\begin{table}[htbp]
  \centering
  \caption{
  Overview of the selections for the $\DMlow$ and $\DMhigh$ signal regions as well as the associated control and validation regions. The control regions include the semi-leptonic \ttbar\ control region (T1LCR), the dileptonic \ttbar\ control region (T2LCR), the $W$+jets control region (WCR), and the single-top $Wt$ control region (STCR).  The validation regions include the semi-leptonic \ttbar\ validation region (T1LVR), the dileptonic \ttbar\ validation region (T2LVR), and the $W$+jets validation region (WVR). List values are provided in between parentheses and square brackets denote intervals. 
  The veto on the reclustered hadronic top-quark candidate is satisfied for events where no reclustered jet candidate is found, or where the mass of the hadronic top-quark (\mTopRecluster) is below a certain threshold. For the WCR, $\DeltaR$($b_1$,$b_2$) $<1.2$ is not required when the event has only one $b$-tagged jet.
  The selection of the $\ttbar+Z$ control region (TZCR) is detailed in Section~\ref{subsec:ttZ}.
  }
  \vspace{3mm}
{\footnotesize
{\renewcommand{\arraystretch}{1.1}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}| l | ccccc |}
                \hline \hline
                                       & \DMlow        & T1LCR/VR             & T2LCR/VR         & WCR/VR                & STCR \\ \hline
                Preselection                            & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge4$,~$\ge1$)  & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge1$) & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge2$) \\
    Jet $\pt$  \,[\GeV]       & \multicolumn{5}{ c |}{$(120~85~65~60)$} \\
    \hline
    \met \,[\GeV]                     & $>320$       & $>250$              & $>230$           & $>250$               & $>250$ \\
    \mt \,[\GeV]                       & $>170$       & $[30,90]$ / $[90,120]$ & $>120$           & $[30,90]$ / $[90,120]$ & $[30,120]$ \\
    \HTmissSig                        & $>14$       & $>10$              & $>10$            & $>10$                & $>10$ \\
    \mTopRecluster \,[\GeV]                 & $>130$       & $>130$               & top veto / $>130$  & top veto             & top veto \\
    \amtTwo \,[\GeV]                        & $>160$       & $<200$               & $<160$           & $>160$               & $>200$ \\
    \dPMETlep                        & $>1.2$        & --                   & $>1.2$         & --                   & -- \\
    \minDeltaPhi                & $>1.0$        & --              & --               & --                   & -- \\
    $\DeltaR(b,\ell)$              & $<2.0$       & --                   & --               & --                   & -- \\
    $\DeltaR$($b_1$,$b_2$)             & --               & --                   & --               & $<1.2$               & $>1.2$ \\
    Lepton charge                     & --             & --              & --               & $+1$                 & -- \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{5}{ c |}{$>0.4$}                  \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]   & \multicolumn{5}{ c |}{$>80$}                   \\ 
    \hline \hline
                                       & \DMhigh        & T1LCR/VR       & T2LCR/VR         & WCR                & STCR \\ \hline
                Preselection                            & \multicolumn{5}{ c |}{high-\met\ preselection} \\ \hline
    Number of (jets,~$b$-tags)     & ($\ge4$,~$\ge1$)  & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge1$) & ($\ge4$,~$\ge1$)     & ($\ge4$,~$\ge2$) \\
    Jet $\pt$ \,[\GeV]       & \multicolumn{5}{ c |}{$(125~75~65~25)$} \\
    \hline
    \met \,[\GeV]                     & $>380$       & $>280$              & $>280$           & $>280$               & $>280$ \\
    \mt \,[\GeV]                       & $>225$       & $[30,90]$ / $[90.120]$ & $>120$           & $[30,90]$ / $[90,120]$ & $[30,120]$ \\
    \mTopRecluster \,[\GeV]                 & $>130$       & $>130$               & top veto / $>130$  & top veto             & top veto \\
    \amtTwo \,[\GeV]                        & $>190$       & $<200$               & $<200$ / $<190$    & $>190$               & $>200$ \\
    \dPMETlep                        & $>1.2$        & --                   & $>1.2$         & --                   & -- \\
    \minDeltaPhi                & $>1.0$        & $>1.0$              & --               & $>1.0$               & -- \\
    $\DeltaR(b,\ell)$              & $<2.0$       & --                   & --               & --                   & -- \\
    $\DeltaR$($b_1$,$b_2$)             & --               & --                   & --               & $<1.2$               & $>1.2$ \\
    Lepton charge                     & --             & --              & --               & $+1$                 & -- \\
        $|\Delta\phi(j_{1,2},\Ptmiss)|$          & \multicolumn{5}{ c |}{$>0.4$}                  \\ 
        $\mtTwoTau$ based $\tau$-veto\,[\GeV]   & \multicolumn{5}{ c |}{$>80$}                   \\ 
    \hline \hline
  \end{tabular*}
}
}
  \label{tab:CRs_DM}
\end{table}

